Feedback vertex sets in oriented graphs

For an oriented graph $G$, denote by $fvs(G)$ the minimum number of vertices whose deletion from $G$ makes it acyclic. We show that an oriented graph $G$ on $n$ vertices and $m$ arcs satisfies $fvs(G) \le \frac{2n+m+h}{9}$ where $h$ denotes the number of connected components of $G$ that belong to a special class of oriented graphs. This result has three consequences. First, when $G$ is planar, we obtain that $fvs(G) \le \frac{2n+m}{9}$. In particular, this implies that $fvs(G) \le \frac{5n-6}{9}$ for any planar oriented graph $G$, improving the best known upper bound of $\frac{3n}{5}$~[Borodin, Discrete Mathematics, 1979]. Then, applying this inequality to the planar digraphs without directed triangles, we get that $fvs(G) \le \frac{6n-8}{13}$, which improves the current best bound of $\frac{n}{2}$~[Li and Mohar, SIAM Journal on Discrete Mathematics, 2017]. Finally, when $G$ has maximum degree 6, we have $fvs(G) \le \frac{4n}{7}$ and this bound is tight, answering a conjecture of Ai, Gutin, Liu, Yeo and Zhou~[arXiv:2512.01676, 2025].

==> preamble.tex <==
\ProvidesFile{preamble.tex}


% Packages -----------------------------------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage[table]{xcolor}
\usepackage{stmaryrd}
\usepackage{bbold}
\usepackage{multirow}
\usepackage{geometry}



% Packages du template de base ----------------------------------------------------------------
\usepackage{microtype}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{caption}
\captionsetup{belowskip=0pt,aboveskip=0pt}
\usepackage{subcaption}

\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{float}
\usepackage[shortlabels]{enumitem}
\usepackage{hyperref,cleveref,cite,url}
\hypersetup{
 colorlinks,
 citecolor=green!50!black,
 linkcolor=red,
 urlcolor=blue!50!black}

\usepackage{pgf,tikz}

\usepackage{tkz-graph}
\usetikzlibrary{arrows.meta,decorations.markings,bbox,snakes,shapes.misc}


\tikzset{
  decoration={snake},
  cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
  ->-/.style={decoration={
      markings,
      mark=at position #1 with {\arrow{>}}
    },postaction={decorate}},
  ->-/.default=0.55 % default position for the arrow on edges
}

\usetikzlibrary{automata}
\usetikzlibrary{patterns}

\usetikzlibrary{backgrounds,calc,positioning}
\usepackage{authblk}


\geometry{hmargin=1.5cm,vmargin=1.5cm}


% Numerotation des sections et indentation --------------------------------------------------------------

\parindent 0mm
\parskip 3mm

\setenumerate{label=\textup{(\arabic*)}, noitemsep, topsep=-\parskip, labelindent=.2em, leftmargin=*}
\setitemize{noitemsep, topsep=-\parskip, labelindent=.2em, leftmargin=*}



\setlist[itemize]{label=$\bullet$}


\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim}{Claim}[theorem]
\renewcommand{\theclaim}{\thetheorem.\arabic{claim}}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{application}[theorem]{Application}
\newcommand*{\myproofname}{Proof}
\newenvironment{claimproof}[1][\myproofname]{\begin{proof}[#1]\renewcommand*{\qedsymbol}{\(\diamondsuit\)}}{\end{proof}}
\crefname{conjecture}{Conjecture}{Conjectures}




\newcommand{\NN}[0]{\mathbb{N}}
\newcommand{\IntSet}[2]{\left \llbracket #1 ; #2 \right \rrbracket}
\newcommand{\Modul}[1]{\left | #1 \right |}
\newcommand{\Ent}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\Set}[2]{\left \lbrace #1 \; | \; #2 \right \rbrace}
\DeclareMathOperator{\mult}{mult}
\newcommand{\fa}{fas}
\newcommand{\fv}{fvs}

\DeclareMathOperator{\Root}{Root}
\DeclareMathOperator{\Ch}{Ch}

\renewcommand{\deg}{d}
\newcommand{\degout}{d^{+}}
\newcommand{\degin}{d^{-}}

\makeatletter
\newcommand{\segmentval}[2]{%
  \@ifnextchar\bgroup
    {\segmentval@witharg{#1}{#2}}
    {\delta_{#1}^{#2}}%
}
\newcommand{\segmentval@witharg}[3]{\delta_{#1}^{#2}(#3)}
\makeatother

